SceneWright: Benchmarking Coding Agents on Multi-View Procedural 3D Modeling of Outdoor Scenes

Can a coding agent reconstruct an outdoor scene in code from calibrated views? We study multi-view procedural 3D modeling, in which an agent writes Blender code to build class-labeled entities in the metric frame of posed cameras. Existing evaluations fall short in this setting: scoring 2D rendered views can hide flawed 3D geometry, while aligning predicted meshes to ground truth leaves pose and scale untested. We introduce SceneWright, a benchmark of 50 script-built outdoor scenes paired with exact Blender ground truth. Each scene is posed as both a sparse-view image task and a dense survey-video task, for 100 tasks in total. Submitted scenes are scored directly against ground truth across four dimensions: layout, semantic composition, and geometric and visual fidelity. We test 11 models, each under its vendor CLI and under OpenCode, for 22 configurations. Our results show that the underlying model largely dictates the performance tier, while the effect of the agent harness varies from model to model, and higher token spend does not translate to better reconstructions. Agents differ far more in metric structure than in surface appearance, and under the current interface they gain little from a dense survey video over sparse views, using under 1% of its frames. Finally, turning the inspection, iterative refinement, and photogrammetric practices of top-performing agents into harness skills lifts two weaker models without weight updates, pointing to the harness as a lever worth exploring.

==> cover/assets/bg_cover_frost_geom.tex <==
\def\swc@bgw{612.000}\def\swc@bgh{379.247}
\def\swc@bgboardx{98.000}\def\swc@bgboardy{50.734}
\def\swc@bgboardw{416.000}\def\swc@bgboardh{267.740}
\endinput


==> cover/cover.tex <==
\RequirePackage{fix-cm}%
\RequirePackage{xcolor}
\RequirePackage{graphicx}
\RequirePackage{tikz}
\edef\swcoverRestoreAtCatcode{\catcode64=\the\catcode64\relax}
\input{cover/sw-tokens}%
\catcode64=11\relax

\providecommand\swcoverassets{cover/assets}
\providecommand\swcoverbg{\swcoverassets/bg_cover_frost.png}
\def\swc@file@abstract{cover/abstract_body.tex}
\def\swc@file@logo{cover/assets/SceneWright_logo.png}
\def\swc@file@board{\swcoverassets/leaderboard.pdf}
\def\swc@file@bg{\swcoverbg}
\@namedef{swc@icon@homepage}{cover/assets/icon_globe_accent.pdf}
\@namedef{swc@icon@huggingface}{cover/assets/icon_huggingface.pdf}
\@namedef{swc@icon@github}{cover/assets/icon_github_accent.pdf}
\@namedef{swc@label@homepage}{Homepage}
\@namedef{swc@label@huggingface}{Hugging Face}
\@namedef{swc@label@github}{GitHub}
\def\swc@placeholder{}%
\def\swc@boardtitle{Leaderboard}
\def\swc@boarddesc{Overall score $J$ of the 22 model + harness configurations on the 100 tasks,
  each bar split into the shares of $\bar{E}_1$--$\bar{E}_4$.}

\def\swc@margin{54}      %
\def\swc@top{28}         %
\def\swc@bottom{24}      %
\def\swc@gap{8}          %
\def\swc@radius{7.09}    %
\def\swc@padx{20}        %
\def\swc@padt{11}        %
\def\swc@padb{11}        %
\def\swc@bpadx{13}       %
\def\swc@bpadt{11}       %
\def\swc@bpadb{9}        %
\def\swc@bmin{11}        %
\def\swc@bgtol{0.5}      %
\def\swc@titlesize{34}   \def\swc@logoh{51}   \def\swc@logogap{11}%
\def\swc@subsize{16.5}   \def\swc@sublead{20}%
\def\swc@authsize{9}     \def\swc@authlead{11.5}%
\def\swc@affsize{10}     \def\swc@afflead{12.5}
\def\swc@cornerlogow{77}%
\def\swc@cornerpos{1}  %
\def\swc@headtop{14}    %
\def\swc@headgap{12}    %
\def\swc@instlogoh{26.4} \def\swc@instlogogap{16}%
\def\swc@affcolumns{0}  %
\def\swc@affcolgap{22}    \def\swc@afflogogap{5}%
\def\swc@abssize{9.75}   \def\swc@abslead{12.4}
\def\swc@linksize{9.1}   \def\swc@iconh{10}
\def\swc@btitlesize{10.5}
\def\swc@bdescsize{9.1}

\def\swc@title{}\def\swc@subtitle{}
\newcount\swc@nauth \newcount\swc@naff \newcount\swc@nlink \newcount\swc@i
\def\swtitle#1{\gdef\swc@title{#1}}
\def\swsubtitle#1{\gdef\swc@subtitle{#1}}
\def\swauthor{\@ifnextchar[\swc@author{\swc@author[]}}
\def\swc@author[#1]#2{\global\advance\swc@nauth\@ne
  \expandafter\gdef\csname swc@au@\the\swc@nauth\endcsname{#2}%
  \expandafter\gdef\csname swc@aum@\the\swc@nauth\endcsname{#1}}
\def\swaffiliation{\@ifnextchar[\swc@affil{\swc@affil[]}}
\def\swc@affil[#1]#2#3{\global\advance\swc@naff\@ne
  \if\relax\detokenize{#1}\relax
    \expandafter\xdef\csname swc@afm@\the\swc@naff\endcsname{\the\swc@naff}%
  \else
    \expandafter\gdef\csname swc@afm@\the\swc@naff\endcsname{#1}%
  \fi
  \expandafter\gdef\csname swc@af@\the\swc@naff\endcsname{#2}%
  \expandafter\gdef\csname swc@afl@\the\swc@naff\endcsname{#3}}
\def\swc@cornerlogo{}
\def\swcornerlogo#1{\gdef\swc@cornerlogo{#1}}
\def\swlink#1#2{\global\advance\swc@nlink\@ne
  \expandafter\xdef\csname swc@lk@\the\swc@nlink\endcsname{\detokenize{#1}}%
  \expandafter\gdef\csname swc@lu@\the\swc@nlink\endcsname{#2}}

\newsavebox\swc@upperbox \newsavebox\swc@boardbox \newsavebox\swc@tmpbox
\def\swc@hvscale{1}
\def\swc@sf#1#2{\fontsize{\strip@pt\dimexpr #1bp*65536/\number\dimexpr\swc@hvscale pt\relax\relax}%
  {#2bp}\selectfont}
\def\swc@rm#1#2{\fontsize{\strip@pt\dimexpr #1bp\relax}{#2bp}\selectfont}
\def\swc@balanced{\leftskip=\z@ plus 0.3\hsize \rightskip=\leftskip \parfillskip=\z@
  \hyphenpenalty=\@M \exhyphenpenalty=\@M \pretolerance=\m@ne \tolerance=\@M \hbadness=\@M
  \spaceskip=\fontdimen2\font \xspaceskip=\fontdimen2\font}
\def\swc@vgap#1{\par\nointerlineskip\vskip #1bp\relax}
\def\swc@ifempty#1{\if\relax\detokenize\expandafter{#1}\relax\expandafter\@firstoftwo
  \else\expandafter\@secondoftwo\fi}
\def\swc@capcenter#1{\setbox\z@\hbox{#1}\raise\dimexpr 0.5\fontcharht\font`H-0.5\ht\z@\relax\box\z@}

\def\swc@authors{%
  \swc@i=\z@
  \loop\ifnum\swc@i<\swc@nauth \advance\swc@i\@ne
    \ifnum\swc@i>\@ne \hskip 1.1em plus 0.4em\relax\fi
    \mbox{\csname swc@au@\the\swc@i\endcsname
      \ifnum\swc@naff>\@ne
        \expandafter\swc@ifempty\expandafter{\csname swc@aum@\the\swc@i\endcsname}{}%
          {\textsuperscript{\csname swc@aum@\the\swc@i\endcsname}}%
      \fi}%
  \repeat}
\def\swc@affiliations{%
  \swc@i=\z@
  \loop\ifnum\swc@i<\swc@naff \advance\swc@i\@ne
    \ifnum\swc@i>\@ne \hskip 1.4em plus 0.4em\relax\fi
    \mbox{\ifnum\swc@naff>\@ne\textsuperscript{\csname swc@afm@\the\swc@i\endcsname}\fi
      \csname swc@af@\the\swc@i\endcsname}%
  \repeat}
\def\swc@logos{%
  \swc@i=\z@ \let\swc@sep\relax
  \loop\ifnum\swc@i<\swc@naff \advance\swc@i\@ne
    \expandafter\swc@ifempty\expandafter{\csname swc@afl@\the\swc@i\endcsname}{}{%
      \swc@sep\let\swc@sep\swc@logosep
      \includegraphics[height=\swc@instlogoh bp]{\csname swc@afl@\the\swc@i\endcsname}}%
  \repeat}
\def\swc@logosep{\hskip\swc@instlogogap bp\relax}
\def\swc@affcell#1{{%
  \setbox\z@\hbox{\ifnum\swc@naff>\@ne\textsuperscript{\csname swc@afm@#1\endcsname}\fi
    \csname swc@af@#1\endcsname}%
  \expandafter\swc@ifempty\expandafter{\csname swc@afl@#1\endcsname}%
    {\setbox\tw@\hbox{}}%
    {\setbox\tw@\hbox{\includegraphics[height=\swc@instlogoh bp]{\csname swc@afl@#1\endcsname}}}%
  \dimen@=\wd\z@ \ifdim\wd\tw@>\dimen@ \dimen@=\wd\tw@ \fi
  \vtop{\hbox to\dimen@{\hss\box\z@\hss}\nointerlineskip\vskip\swc@afflogogap bp\relax
    \hbox to\dimen@{\hss\box\tw@\hss}}}}
\def\swc@affcols{%
  \swc@i=\z@
  \loop\ifnum\swc@i<\swc@naff \advance\swc@i\@ne
    \ifnum\swc@i>\@ne \hskip\swc@affcolgap bp\relax\fi
    \swc@affcell{\the\swc@i}%
  \repeat}
\def\swc@haslogos{\@tempswafalse
  \swc@i=\z@
  \loop\ifnum\swc@i<\swc@naff \advance\swc@i\@ne
    \expandafter\swc@ifempty\expandafter{\csname swc@afl@\the\swc@i\endcsname}{}{\@tempswatrue}%
  \repeat}

\def\swc@stripscheme#1://#2\@nil{#2}
\newdimen\swc@labelw \swc@labelw=\z@  %
\def\swc@linklabel{\@ifundefined{swc@label@\swc@key}{\swc@key}{\csname swc@label@\swc@key\endcsname}}
\def\swc@linkitem#1{%
  \edef\swc@key{\csname swc@lk@#1\endcsname}%
  \expandafter\let\expandafter\swc@url\csname swc@lu@#1\endcsname
  \hbox{%
    \@ifundefined{swc@icon@\swc@key}{\ifdim\swc@labelw>\z@\hskip\dimexpr\swc@iconh bp+4.5bp\relax\fi}{%
      \swc@capcenter{\includegraphics[height=\swc@iconh bp]{\csname swc@icon@\swc@key\endcsname}}%
      \hskip 4.5bp\relax}%
    \ifdim\swc@labelw>\z@
      \hbox to\swc@labelw{\bfseries\color{swink}\swc@linklabel\hss}\def\swc@lgap{\hskip 8bp\relax}%
    \else
      {\bfseries\color{swink}\swc@linklabel}\def\swc@lgap{\hskip 5bp\relax}%
    \fi
    \swc@ifempty{\swc@url}%
      {\swc@ifempty{\swc@placeholder}{}{\swc@lgap{\color{swink3}\swc@placeholder}}}%
      {\swc@lgap\@ifundefined{href}{\swc@urltext}{\expandafter\href\expandafter{\swc@url}{\swc@urltext}}}}}
\def\swc@urltext{{\color{swaccent}\ttfamily
  \edef\swc@urlstr{\expandafter\detokenize\expandafter{\swc@url}}%
  \expandafter\in@\expandafter{\detokenize{://}}{\swc@urlstr}%
  \ifin@\expandafter\swc@stripscheme\swc@urlstr\@nil\else\swc@urlstr\fi}}
\def\swc@linksep{\hskip 11bp\relax{\color{swrule}\vrule width 0.6bp height 7.6bp depth 1.6bp}%
  \hskip 11bp\relax}
\def\swc@linkrow{%
  \swc@i=\z@ \let\swc@sep\relax
  \loop\ifnum\swc@i<\swc@nlink \advance\swc@i\@ne
    \swc@sep\let\swc@sep\swc@linksep
    \swc@linkitem{\the\swc@i}%
  \repeat}
\def\swc@linkstack{%
  \swc@i=\z@
  \loop\ifnum\swc@i<\swc@nlink \advance\swc@i\@ne
    \edef\swc@key{\csname swc@lk@\the\swc@i\endcsname}%
    \setbox\z@\hbox{\bfseries\swc@linklabel}%
    \ifdim\wd\z@>\swc@labelw \swc@labelw=\wd\z@ \fi
  \repeat
  \swc@i=\z@
  \hbox to\hsize{\hss\vbox{\baselineskip=1.45em
    \loop\ifnum\swc@i<\swc@nlink \advance\swc@i\@ne
      \hbox{\swc@linkitem{\the\swc@i}}%
    \repeat}\hss}}

\def\swc@buildupper{%
  \setbox\swc@upperbox\vbox{%
    \hsize=\dimexpr\swc@cardw bp-2\dimexpr\swc@padx bp\relax\relax
    \linewidth=\hsize \parindent=\z@ \parskip=\z@ \leftskip=\z@ \rightskip=\z@
    \parfillskip=\z@ plus 1fil\relax \everypar{}\color{swink}%
    \hbox to\hsize{\hss
      \swc@sf{\swc@titlesize}{\swc@titlesize}\sffamily\bfseries
      \swc@capcenter{\includegraphics[height=\swc@logoh bp]{\swc@file@logo}}%
      \hskip\swc@logogap bp\relax
      {\color{swaccent}\swc@title}\hss}%
    \swc@vgap{4}%
    {\swc@sf{\swc@subsize}{\swc@sublead}\sffamily\bfseries\swc@balanced\color{swink}\swc@subtitle\par}%
    \swc@vgap{10}%
    {\swc@sf{\swc@authsize}{\swc@authlead}\sffamily\swc@balanced\color{swink}\swc@authors\par}%
    \swc@vgap{4}%
    \swc@haslogos
    \ifnum\swc@affcolumns=\z@ \@tempswafalse \fi
    \if@tempswa
      {\rmfamily\swc@rm{\swc@affsize}{\swc@afflead}\color{swink2}%
       \hbox to\hsize{\hss\swc@affcols\hss}}%
    \else
      {\rmfamily\swc@rm{\swc@affsize}{\swc@afflead}\swc@balanced\color{swink2}\swc@affiliations\par}%
      \swc@haslogos
      \if@tempswa\swc@vgap{7}\hbox to\hsize{\hss\swc@logos\hss}\fi
    \fi
    \swc@vgap{11}%
    {\rmfamily\swc@rm{\swc@abssize}{\swc@abslead}\color{swink}\emergencystretch=1em
     \input{\swc@file@abstract}\par}%
    \ifnum\swc@nlink>\z@
      \swc@vgap{8}%
      {\color{swrule}\hrule height 0.4bp}%
      \swc@vgap{7}%
      {\swc@sf{\swc@linksize}{12}\sffamily\color{swink}%
       \setbox\swc@tmpbox\hbox{\swc@linkrow}%
       \ifdim\wd\swc@tmpbox>\hsize \swc@linkstack \else\hbox to\hsize{\hss\box\swc@tmpbox\hss}\fi}%
    \fi}}

\def\swc@buildboard{%
  \setbox\swc@tmpbox\hbox{\includegraphics{\swc@file@board}}%
  \setbox\swc@boardbox\vbox{%
    \hsize=\wd\swc@tmpbox \parindent=\z@ \parskip=\z@ \leftskip=\z@ \rightskip=\z@
    \parfillskip=\z@ plus 1fil\relax \everypar{}%
    \hbox{\swc@sf{\swc@btitlesize}{12}\sffamily\bfseries\color{swaccent}\swc@boardtitle}%
    \swc@vgap{3.5}%
    {\rmfamily\swc@rm{\swc@bdescsize}{11}\color{swink2}%
     \setbox\z@\hbox{\swc@boarddesc}%
     \ifdim\wd\z@>\hsize \swc@boarddesc\par \else \box\z@ \fi}%
    \swc@vgap{7}%
    \box\swc@tmpbox}}

\newcommand\makecover{%
  \begingroup
  \@ifundefined{Hv@scale}{\def\swc@hvscale{1}}{\edef\swc@hvscale{\Hv@scale}}%
  \pgfmathsetmacro\swc@pw{\paperwidth/1bp}\pgfmathsetmacro\swc@ph{\paperheight/1bp}%
  \pgfmathsetmacro\swc@L{\swc@margin}\pgfmathsetmacro\swc@R{\swc@pw-\swc@margin}%
  \pgfmathsetmacro\swc@cardw{\swc@R-\swc@L}%
  \swc@buildupper
  \swc@buildboard
  \swc@ifempty{\swc@cornerlogo}{}{%
    \ifnum\swc@cornerpos=\@ne
      \setbox\z@\hbox{\includegraphics[width=\swc@cornerlogow bp]{\swc@cornerlogo}}%
      \pgfmathsetmacro\swc@top{\swc@headtop+(\ht\z@+\dp\z@)/1bp+\swc@headgap}%
    \fi}%
  \pgfmathsetmacro\swc@Yone{\swc@top+\swc@padt+(\ht\swc@upperbox+\dp\swc@upperbox)/1bp+\swc@padb}%
  \pgfmathsetmacro\swc@Ytwo{\swc@Yone+\swc@gap}%
  \pgfmathsetmacro\swc@B{\swc@ph-\swc@bottom}%
  \pgfmathsetmacro\swc@Hl{\swc@B-\swc@Ytwo}%
  \pgfmathsetmacro\swc@cx{\swc@pw/2}%
  \pgfmathsetmacro\swc@cy{(\swc@Ytwo+\swc@B)/2}%
  \pgfmathsetmacro\swc@bw{\wd\swc@boardbox/1bp+2*\swc@bpadx}%
  \pgfmathsetmacro\swc@bh{(\ht\swc@boardbox+\dp\swc@boardbox)/1bp+\swc@bpadt+\swc@bpadb}%
  \pgfmathsetmacro\swc@bs{min(1,(\swc@Hl-2*\swc@bmin)/\swc@bh,(\swc@cardw-2*\swc@bmin)/\swc@bw)}%
  \pgfmathparse{\swc@bs<1}%
  \ifnum\pgfmathresult=1
    \PackageWarningNoLine{cover}{The leaderboard with its frosted zone (\swc@bw\space x \swc@bh\space
      bp) does not fit its region (\swc@cardw\space x \swc@Hl\space bp) with \swc@bmin\space bp
      around it; it is scaled by \swc@bs, and the frosted zone of the scene no longer matches it.
      Shorten the upper card or regenerate the board smaller}%
    \pgfmathsetmacro\swc@bw{\swc@bw*\swc@bs}\pgfmathsetmacro\swc@bh{\swc@bh*\swc@bs}%
  \fi
  \pgfmathsetmacro\swc@bx{\swc@cx-\swc@bw/2}\pgfmathsetmacro\swc@by{\swc@cy-\swc@bh/2}%
  \pgfmathsetmacro\swc@ix{\swc@bx+\swc@bs*\swc@bpadx}\pgfmathsetmacro\swc@iy{\swc@by+\swc@bs*\swc@bpadt}%
  \pgfmathsetmacro\swc@biw{\wd\swc@boardbox/1bp}%
  \pgfmathsetmacro\swc@bih{(\ht\swc@boardbox+\dp\swc@boardbox)/1bp}%
  \pgfmathparse{abs(\swc@biw-\swc@bgboardw)>\swc@bgtol || abs(\swc@bih-\swc@bgboardh)>\swc@bgtol}%
  \ifnum\pgfmathresult=1
    \PackageWarningNoLine{cover}{The leaderboard block is \swc@biw\space x \swc@bih\space bp, but
      the scene \swc@file@bg\space was made for \swc@bgboardw\space x \swc@bgboardh\space bp: its
      frosted zone no longer fits the board. Regenerate the scene with make_bg_cover.py --board
      \swc@biw\space \swc@bih}%
  \fi
  \pgfmathsetmacro\swc@gx{\swc@ix-\swc@bgboardx}\pgfmathsetmacro\swc@gy{\swc@iy-\swc@bgboardy}%
  \typeout{SWCOVER: upper card y=\swc@top-\swc@Yone, x=\swc@L-\swc@R; board region
    y=\swc@Ytwo-\swc@B; frosted zone x=\swc@bx+\swc@bw, y=\swc@by+\swc@bh; board block
    x=\swc@ix+\swc@biw, y=\swc@iy+\swc@bih, scale \swc@bs; scene PNG x=\swc@gx+\swc@bgw,
    y=\swc@gy+\swc@bgh (bp from the top left)}%
  \thispagestyle{empty}%
  \par\noindent
  \begin{tikzpicture}[remember picture,overlay]
    \begin{scope}[shift={(current page.north west)},x=1bp,y=-1bp]
      \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (\swc@gx,\swc@gy)
        {\includegraphics[width=\swc@bgw bp]{\swc@file@bg}};
      \fill[swtint,rounded corners=\swc@radius bp] (\swc@L,\swc@top) rectangle (\swc@R,\swc@Yone);
      \node[anchor=north,inner sep=0pt,outer sep=0pt] at (\swc@cx,\swc@top+\swc@padt)
        {\usebox\swc@upperbox};
      \swc@ifempty{\swc@cornerlogo}{}{%
        \ifnum\swc@cornerpos=\@ne
          \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (\swc@L,\swc@headtop)
            {\includegraphics[width=\swc@cornerlogow bp]{\swc@cornerlogo}};
        \else
          \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (\swc@L+\swc@padx,\swc@top+\swc@padt)
            {\includegraphics[width=\swc@cornerlogow bp]{\swc@cornerlogo}};
        \fi}%
      \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (\swc@ix,\swc@iy)
        {\scalebox{\swc@bs}{\usebox\swc@boardbox}};
    \end{scope}
  \end{tikzpicture}%
  \par
  \endgroup
  \clearpage}

\def\swc@pngstem#1.png#2\@nil{#1}
\edef\swc@file@geom{\swc@file@bg}
\edef\swc@file@geom{\expandafter\swc@pngstem\swc@file@geom.png\@nil _geom.tex}
\input{\swc@file@geom}

\swcoverRestoreAtCatcode
\endinput


==> cover/sw-tokens.tex <==
\makeatletter
\@ifpackageloaded{xcolor}{}{\PackageError{sw-tokens}{Load xcolor before cover/sw-tokens.tex}{}}
\makeatother
\definecolor{swaccent}{HTML}{2E5AA8}   %
\definecolor{swtint}{HTML}{EEF2F8}     %
\definecolor{swink}{HTML}{1D2633}      %
\definecolor{swink2}{HTML}{3B4656}     %
\definecolor{swink3}{HTML}{6B7686}     %
\definecolor{swrule}{HTML}{C9D1DA}     %
\definecolor{swE1}{HTML}{607BBC}       %
\definecolor{swE2}{HTML}{26A7C8}       %
\definecolor{swE3}{HTML}{65C4B9}       %
\definecolor{swE4}{HTML}{A4D3B7}       %
\definecolor{swvendor}{HTML}{337BAC}   %
\definecolor{swopencode}{HTML}{4FB1B2} %
\definecolor{swband}{HTML}{F1F5F9}     %
\definecolor{swaxis}{HTML}{A9B3BF}     %

